Carbon Explorer: A Holistic Approach for Designing Carbon Aware Datacenters

Technology companies have been leading the way to a renewable energy transformation, by investing in renewable energy sources to reduce the carbon footprint of their datacenters. In addition to helping build new solar and wind farms, companies make power purchase agreements or purchase carbon offsets, rather than relying on renewable energy every hour of the day, every day of the week (24/7). Relying on renewable energy 24/7 is challenging due to the intermittent nature of wind and solar energy. Inherent variations in solar and wind energy production causes excess or lack of supply at different times. To cope with the fluctuations of renewable energy generation, multiple solutions must be applied. These include: capacity sizing with a mix of solar and wind power, energy storage options, and carbon aware workload scheduling. However, depending on the region and datacenter workload characteristics, the carbon-optimal solution varies. Existing work in this space does not give a holistic view of the trade-offs of each solution and often ignore the embodied carbon cost of the solutions. In this work, we provide a framework, Carbon Explorer, to analyze the multi-dimensional solution space by taking into account operational and embodided footprint of the solutions to help make datacenters operate on renewable energy 24/7. The solutions we analyze include capacity sizing with a mix of solar and wind power, battery storage, and carbon aware workload scheduling, which entails shifting the workloads from times when there is lack of renewable supply to times with abundant supply.

==> todos.tex <==


- Include Advanced Battery model
- Emphasize the last 5-10\% in 24/7 is really hard
- Present as a configurable/flexible framework
- Mention Carbon Explorer can help guide DC site selection
- Include technical details on the framework
- Adding use cases of the framework, who and how are they going to use it
- Skipping Grid mix, hybrid regions to shorten

+ Figure 15: add labels of optimal renewable coverage
+ Mentioned UN's 24/7 Compact,
   24/7 commitments of Google/Microsoft not cited not to reveal the paper is from Meta
